Direct Evaluation of Chain-of-Thought in Multi-hop Reasoning with Knowledge Graphs

Large language models (LLMs) demonstrate strong reasoning abilities when prompted to generate chain-of-thought (CoT) explanations alongside answers. However, previous research on evaluating LLMs has solely focused on answer accuracy, neglecting the correctness of the generated CoT. In this paper, we delve deeper into the CoT reasoning capabilities of LLMs in multi-hop question answering by utilizing knowledge graphs (KGs). We propose a novel discriminative and generative CoT evaluation paradigm to assess LLMs' knowledge of reasoning and the accuracy of the generated CoT. Through experiments conducted on 5 different families of LLMs across 2 multi-hop question-answering datasets, we find that LLMs possess sufficient knowledge to perform reasoning. However, there exists a significant disparity between answer accuracy and faithfulness of the CoT reasoning generated by LLMs, indicating that they often arrive at correct answers through incorrect reasoning.

==> figures/num_step.tex <==
\begin{figure*}
   \centering
   \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
        \includegraphics[width=8cm]{images/CWQ_num_step.pdf}
        &
        \includegraphics[width=8cm]{images/GrailQA_num_step.pdf}
    \end{tabular}
    } 
    \caption{The average of the number of reasoning steps of LLMs on datasets. Standard denotes the average number of steps in the ground truth reasoning paths.}
    \label{fig:num_step} 
\end{figure*}

==> sections/2-background_old.tex <==
\section{Preliminaries}
\subsection{Chain-of-thought}
https://arxiv.org/pdf/2311.11797.pdf
Fewshot CoT

\subsection{Knowledge Graph}


\subsection{ Notation and Definitions}\label{Formulation}
We first formally define the concepts of a step-by-step reasoning response in the context of our framework. 

\textbf{A reasoning step} $s$ is a sentence responding to an index in a numbered list in LLM response. \reza{do we assume there is only 'one' KG triplet corresponding to a reasoning step in CoT?\vuong{-> yes}\\
Are there cases where there are multiple relations mentioned in a reasoning step of CoT? \vuong{-> From my observation, some cases have multiple relations, however, in our assumption, we only extract the best similarity of relation \& entities}}

\textbf{A KG triple} $T=<h,r,t>$ presenting relation $r$ of the head entity $h$ and the tail entity $t$, is the triple retrieved from KG with highest probability $p$ of the reasoning step $s$. The step is a \textit{factual error} if $p$ is lower than the given threshold $\alpha$, or the ratio of overlap of $h$, $t$ in $s$ is lower than the given threshold $\beta$.

\textbf{A final answer} $a$ is the extracted text from the conclusion sentence which has the format \textit{"So the answer is (<final answer of the question>)."}

\textbf{A CoT response} $A=<S, a>$, where $S=s_1,s_2,...,s_n$ is a sequence of reasoning steps, $a$ is the final answer.

\textbf{A reasoning path} $\mathcal{P}=<T_1,T_2,...,T_n>$, where $T_i$ is a retrieved triple from KG corresponding to the reasoning step $s_i$ with the highest probability $p_i$. It is correct if it creates a connected graph and no existence of factual error.
This definition is found to be similar to definition 4 of \citet{creswell2022faithful}.

\textbf{A ground truth reasoning path} $\mathcal{GP}=<T_1,T_2,...,T_m>$, provided by a specific dataset or is retrieved from SPARQL provided in the dataset, with $h_0$ is a topic entity and $t_m$ is the ground truth final answer, $h_j=t_{j-1}$.


==> sections/3-method-linhao.tex <==
\section{Evaluating the CoT Reasoning of LLMs}\label{sec:method}
In this section, we introduce the proposed method to evaluate the chain-of-though (CoT) reasoning process of LLMs with the help of knowledge graphs (KGs). Specifically, we propose two evaluation modes: \emph{discriminative evaluation} and \emph{generative evaluation}. The discriminative evaluation aim to investigate whether LLMs possess enough knowledge for conducting valid reasoning and the generative evaluation further analyze whether LLMs can provide valid reasoning process during CoT generation. The overall framework is shown in \Cref{fig:framework}.

\input{figures/framework}

\subsection{Discriminative Evaluation}\label{sec:dis_eval}
The discriminative evaluation aims to analyze whether the LLMs possess enough knowledge for conducting valid reasoning. \nreza{made it more clear, sounds good?} \reza{We hypothesize that 
%
if the LLMs posses sufficient factual knowledge and are capable of faithful reasoning, they should be able to distinguish valid reasoning paths from invalid ones. 
%
%if the LLMs are capable of generating faithful reasoning, they should have sufficient knowledge to discriminate faithful from unfaithful reasoning.
}
Following previous studies that evaluate the factual knowledge inside LLMs \cite{luo-etal-2023-systematic}, we feed both the valid and \reza{invalid} reasoning paths to the LLMs and ask them to predict the validity of these paths. \ctrang{Do we really feed both paths? In the example, we only feed one - either valid or invalid} This allows us to assess the reasoning knowledge inside LLMs by analyzing their prediction accuracy.

We carefully design prompts to describe the task and instruct LLMs to provide the prediction. An example of the zero-shot prompt template is,

\begin{minipage}{0.95\columnwidth}
  \centering
  \vspace{1mm}
  \begin{tcolorbox}[title=Zero-shot Discriminative Evaluation Prompt, fonttitle=\bfseries\small]
      \small
      Given this reasoning path, do you think this is a valid path to answer the question? If yes please answer "YES", otherwise please answer "NO".
      \vspace{5pt}
      \\
      Question:\\
      \texttt{<Question>}
      \vspace{5pt}
      \\
      Reasoning path:\\
      \texttt{<Reasoning Path>}
  \end{tcolorbox}
  \vspace{1mm}
\end{minipage}
where \texttt{<Question>} indicates the question, and \texttt{<Reasoning Path>} denotes the input reasoning path, which is verbalized as a \reza{structured} sentence,
\begin{equation}
  \centering
  e_0\to r_1\to e_1\to \dots \to r_l \to e_l.
\end{equation}

The valid reasoning paths are extracted from the ground-truth reasoning paths\footnote{The ground-truth reasoning paths are constructed from the SPARQL query provided in the datasets. The detailed construction in Appendix \ref{appendix:subgraph_gr_construct}.} $P^*\in\mathcal{P}^*$. \nreza{when we randomly corrupt entites, can we do it in a such a way that the edge before the entity is in KG, but the edge after that is not in the KG (and vice versa)? this makes the invalid paths harder to identify \LH{Yes, when constructing the negative samples, we randomly select the entities to be replaced. Thus, there could be right-than-error, or error-than-right in the negative samples.}} \reza{We  construct  an invalid reasoning path $P'$  by randomly corrupting the entities. This would result in some factual errors in the reasoning path, which are not valid for answering the question. To thoroughly assess the reasoning abilities of LLMs, in addition to the zero-shot prompt, we have also developed few-shot, zero-shot CoT, and few-shot CoT prompts. The details of these prompts are shown in the \todo{Appendix}.}

\noindent\textbf{Findings:} The results of the discriminative assessment are shown in \S\ref{sec:dis_results}. From the results, we can conclude that even LLMs posses enough reasoning knowledge, they still have limitations in performing accurate reasoning during CoT generation. Therefore, we propose the generative evaluation to assess the validity of CoT reasoning in LLMs' generation.

\subsection{Generative Evaluation}\label{sec:gen_eval}
\reza{
The generative evaluation aims to assess the validity (faithfulness) \todo{check to ensure the consistency of terminology} of the CoT reasoning process \emph{generated} by LLMs. 
%
Our main idea is to \emph{ground} LLMs' CoT into KG and verify whether it forms a valid path. 
%
% Evaluating the validity of the reasoning process is challenging due to the unstructured nature of the text generated as the CoT reasoning. We thus propose to convert unstructured CoT reasoning to structured KG-like paths.
}
\trang{To address the challenge of evaluating unstructured CoT, we carefully design a prompting strategy to instruct LLMs to output the CoT in a structured format. This enables us to parse LLM's response into a structured reasoning path, which can then be validated against KG. The example prompts and structured CoT output are provided in \Cref{appendix:gen-prompt}.}

Specifically, given a generated CoT response $S$ of question $q$, we first construct a reasoning path $\hat{P}$ by \reza{retrieving} triples from the KGs. Then we evaluate the validity of the reasoning path by checking whether the path connects the question and answer entities in the KGs. The details of these steps are explained in the following subsections. 

\subsubsection{Reasoning Path Construction}\label{sec:path_construct}
Given a CoT response $S=\{s_1,s_2,\ldots,s_n\}$, we first retrieve a triple\footnote{\todo{We noticed in almost all  cases in our experiments, a CoT step corresponds to one KG triplet. The extension to multiple triplets per CoT step is left for future work. } \reza{please double check. this extension amount to a beautiful problem which i believe has a nice dynamic programming alg }} $T=(e_h,r,e_t)$ for each step $s_i$ in the CoT response.%\footnote{The CoT generation prompts can be found in \todo{Appendix}} 
The retrieved triples are the structural representation of each reasoning step which can be used to construct the reasoning path for evaluation.

Previous works usually retrieve triples by identifying the entities and relations mentioned in the sentence and linking them to the KGs \todo{Cite}. However, this process is burdensome and cannot be applied to large-scale KGs. Inspired by the recent fact retrieval method \cite{baek2023direct}, we represent the reasoning step $s$ and triples in a unified embedding space and retrieve the triple $T$ based on their embedding similarity.  

For all the triples in the KGs, we verbalize each triplet into a sentence \trang{by concatenating the entities and relation} $x="e_h~r~e_t."$. Then we use the Sentence-BERT model \citep{reimers-2019-sentence-bert} to obtain its embedding $h_T=E(x)$. These embeddings are constructed in advance and saved in a vector database FAISS \cite{johnson2019billion} for efficient retrieval. Similarly, the embedding of a given reasoning step $s$ is computed as $h_{s} = E(s)$. Then we retrieve the top-$k$ triples from KG by calculating the embedding similarity between $h_{s}$ and $h_T$ as:
\begin{equation}
  \centering
  \tau_i = f(h_{s}, h_{T_i}), \quad T_i=(e_h,r,e_t)\in \mathcal{G},
\end{equation}
where $\tau_i$ denotes the similarity score of triple $T_i$, and $f(\cdot,\cdot)$ is a non-parametric scoring function that measures the similarity between two embeddings. We adopt the cosine similarity as the scoring function in this work. 

The embedding-based retrieval method may lead to the omission of entities mentioned in the reasoning step. To solve this problem, we also take into account the presence of head and tail entities in the reasoning step \trang{in the scoring function}\footnote{https://github.com/seatgeek/thefuzz}. The final score for each retrieved triple is calculated as,
\begin{equation}
  \centering
  \tilde{\tau_i} = \frac{\tau_i + \epsilon_h + \epsilon_t}{3},
\end{equation}
where $\epsilon_h$ and $\epsilon_t$ represent the \vuong{rate of} existence of head and tail entities in the reasoning step, \vuong{which are in the range from 0 to 1 where 0 is no existence, 1 is a complete match}. The overall retrieval process is presented in\nreza{Alg 1 is for triplet retreival not the path construction. \LH{Should we put the path construction in Alg.1?}} \todo{ \Cref{algo:retrieval}}.

We thus  obtain a set of triples $\mathcal{T}=\{T_1,T_2,\ldots,T_n\}$ for the CoT response $S$. Then, we construct the reasoning path $\hat{P}$ by connecting the triples in $\mathcal{T}$. 


\subsubsection{Reasoning Path Evaluation}\label{sec:reasoning_eval}
By evaluating the constructed reasoning path, we can assess the validity of the CoT reasoning process generated by LLMs. Specifically, we evaluate the validity from two aspects: 1) whether the reasoning path contains any factual errors, and 2) whether the reasoning path is valid. Furthermore, we compare the constructed reasoning path with the ground-truth reasoning paths to provide a fine-grained assessment.

\noindent\textbf{Factual Error Detection.} The factual error in the CoT reasoning indicates that LLM might hallucinate at a reasoning step which violates the factual knowledge in KG. Thus, we cannot retrieve any triples that match the reasoning step. To detect the factual errors, we check whether the final score $\tilde{\tau_i}$ of the retrieved triples is below a threshold $\sigma$.

% \noindent\textbf{Reasoning Error Detection.} 
\noindent\textbf{\trang{Validity of Reasoning Path.}} 
A valid CoT reasoning should be able to answer the question, meanwhile, the conclusion of previous step $s_{i-1}$ should be the prerequisite of the current step $s_i$. By treating the prerequisite as the head entities and the conclusion as the tail entities, we can verify whether the reasoning path $\hat{P}$ connects the question and answer entities in the KG. If $\hat{P}$ successfully connects the question and answer entities, we can conclude that the reasoning path is valid.

\noindent\textbf{Fine-grained Assessment.} In addition to the binary evaluation, we can also provide a fine-grained assessment by comparing the constructed reasoning path $\hat{P}$ with the \nreza{what if there is a ``\emph{set}'' of ground truth paths? \LH{In algorithm 3, we compare with all the possible ground-truth paths and select the highest score.}}\reza{ground-truth reasoning path} $P^*$. We adopt a widely used sequence alignment algorithm - Needleman Wunsch algorithm \citep{needleman1970general}, to compare the constructed reasoning path with the ground-truth reasoning paths. In this way, we can obtain continuous alignment scores (i.e., match rate and edit rate) that indicate how close the constructed reasoning path is to the ground-truth reasoning paths. \trang{If there are multiple ground-truth paths, we report the score against the path with the max match rate.}

The details of the reasoning path evaluation and fine-grained assessment are shown in \Cref{algo:eval} and \Cref{algo:eval_groundtruth}, respectively.

\input{algos/algo-eval}
\input{algos/algo_edit_eval}

\subsection{Evaluation Metrics}

\noindent\textbf{Reasoning Results Accuracy.} Conventional studies evaluate the reasoning results by using the accuracy of answers. In addition to the accuracy, we aim to evaluate the correctness of the reasoning process. Specifically, we provide multi-facet metrics to evaluate the CoT reasoning of LLMs. 

To enable robust and truthful reasoning, recently, many LLMs adopt the guardrail techniques \todo{Cite} to abstain from providing answers when they are uncertain (e.g., "there is insufficient information to determine the answer"). Furthermore, LLMs exhibit different instruction-following capabilities, which might return the CoT response in unstructured format. Thus, we consider both the \emph{abstained} and \emph{unstructured} response in the evaluation. 

The precision is only defined as the accuracy of non-abstained and structured reasoning responses, while the recall is the accuracy of all responses, which are formulated as
\begin{align}
    &\resizebox{.6\columnwidth}{!}{
    $\text{Precision} =\frac{\#\text{correct}}{\#\text{correct}+\#\text{incorrect}},$}\label{eq:precision}\\
    &\resizebox{\columnwidth}{!}{
    $\text{Recall} = \frac{\#\text{correct}}{\#\text{correct}+\#\text{incorrect}+\#\text{abstained}+\#\text{unstructured}},$\label{eq:recall}
    }
\end{align}
where the $\#\text{correct}$ denotes the number of responses containing correct answers.
The F1 score is calculated as $F1=2*\frac{\text{Precision} * \text{Recall}}{\text{Precision} + \text{Recall}}$. The details of abstained and unstructured response detection are shown in \Cref{appendix:abstained}.

\noindent\textbf{Reasoning Process Accuracy.} To consider the abstained and unstructured response, we adopt the same precision and recall shown in \cref{eq:precision} and \cref{eq:recall}, respectively. The correctness of the reasoning path is detected by the method introduced in \Cref{sec:reasoning_eval}.

==> sections/3-method_old.tex <==
\section{Certification of LLMs'  CoT Reasoning }


\subsection{Discriminative Assessment}
The discriminative assessment aims to analyze whether the LLMs possess enough knowledge for conducting valid reasoning. We hypothesize that if the LLMs are capable of conducting faithful reasoning, they should have sufficient knowledge for reasoning.

Following previous studies \cite{luo2023systematic}, we feed both the ground-truth and negative reasoning paths into the LLMs and ask them to predict the validity of these paths. This allows us to assess the reasoning knowledge inside LLMs by analyzing their prediction accuracy.
%
Carefully designed prompts is designed to describe the tasks and instruct the LLMs to provide the prediction. An example of the Zero-shot prompt template is shown as:

\begin{minipage}{0.95\columnwidth}
  \centering
  \vspace{1mm}
  \begin{tcolorbox}[title=Zero-shot Discriminative Evaluation Prompt, fonttitle=\bfseries\small]
      \small
      Given this reasoning path, do you think this is a valid path to answer the question? If yes please answer "YES", otherwise please answer "NO".
      \vspace{5pt}
      \\
      Question:\\
      \texttt{<Question>}
      \vspace{5pt}
      \\
      Reasoning path:\\
      \texttt{<Reasoning Path>}
  \end{tcolorbox}
  \vspace{1mm}
\end{minipage}
where \texttt{<Question>} indicates the question, and \texttt{<Reasoning Path>} denotes the input reasoning path, which is verbalized as a structural sentence:
\begin{equation}
  \centering
  e_0\to r_1\to e_1\to \dots \to r_l \to e_l.
\end{equation}

The valid reasoning paths are extracted from the ground-truth path $p\in\mathcal{GP}$ \LH{We should have a better notation to indicate the ground-truth path.}. We also construct the invalid reasoning path $p'$ as negative samples by randomly corrupting the entities in the ground-truth path. This would result in some factual errors in the reasoning path, which are not valid for answering the question. 

If the LLMs process sufficient knowledge for reasoning, they should be able to distinguish valid reasoning paths from invalid ones. To thoroughly assess the reasoning abilities of LLMs, in addition to the zero-shot prompt, we have also developed few-shot, zero-shot CoT, and few-shot CoT prompts. The details of these prompts are shown in the \todo{Appendix}.

The results of the discriminative assessment are shown in \Cref{sec:dis_results}. From the results, we can conclude that even LLMs posses enough reasoning knowledge, they still have limitations in performing accurate reasoning during CoT generation. Therefore, we propose a framework to evaluate the validity of CoT reasoning in LLM generations.

\subsection{Generative Assessment}
\label{subsec:gen-cert}
\reza{thanks Vu for the initial version of the section. Trang/Linhao: please have a pass to smooth out this section and its subsections} The generative benchmark aims to evaluate the validity of an LLM through both the final answer and reasoning path. We proposed a framework, that first constructs a reasoning path via LLM's response and Knowledge Graphs, then validate the final answer and the reasoning path via ground truths. This section is structured into four primary components: firstly defining concepts in the context of our framework (\$\ref{Formulation}); then depicting how to generate structured answers (\$\ref{LLMgeneration}); the next part shows the retrieval algorithm and transform LLM response into list of triples (\$\ref{retrieval}), finally evaluation algorithm we proposed to certify LLM answers and reasoning paths(\$\ref{path_eval}).


\subsubsection{LLM answer generation}\label{LLMgeneration}
Given question $Q$, the stage aims to generate a structured CoT response $A$ to construct a reasoning path in the next stage.

\reza{similar to the prompt box that is in section 3.1 for discriminative evaluation, it would be good to havea box for prompting in the generative evaluation mode. } \vuong{-> thanks reza, you updated in appendix \ref{appendix:prompt}} We carefully design a prompt and in-context exemplars to instruct LLMs to produce CoT in a desirable format. It enables automatic parsing into reasoning steps. In particular,\\
Inspired by the Auto-CoT technique proposed \citet{zhang2023automatic}, we utilized zero-CoT prompting and LLM responses to design our fewshot CoT prompt. However, there are a few differences from \citet{zhang2023automatic}:
\begin{itemize}
    \item We directly select examples by categorizing the dataset based on the number of reasoning steps, the number of answers, and types of questions due to apparent characteristics of knowledge base question answering \citep{Talmor2018TheWA}, instead of selecting exemplars based on additional clustering algorithm impacted by algorithm quality.
    \item To obtain better LLM responses, we utilize the APE technique proposed by \citet{zhou2022large}, which demonstrated to outperform the prompt \textit{"Let's think step by step"} \citep{NEURIPS2022_8bb0d291} as \citet{zhang2023automatic} used.
    \item To guarantee the quality of the prompt, we recheck LLM responses for each demonstration based on ground truth reasoning paths accordingly to ensure to match both relation and entities.
\end{itemize}
After this process, the prompt contains a set of 5 demonstrations, which are depicted in prompt \ref{fig:fewshot_cot_only_prompt}.

\subsubsection{Reasoning path construction}\label{retrieval}
For each step $s$ obtained from the structured CoT response $A$, we conduct to transform from LLM-style sentence into the best representative KG triplet $T$. 

\input{algos/algo-retrieval}

The transformation method is shown in \cref{algo:retrieval}. Triples $T=<h,r,t>$ from KG are verbalized into sentences format $"\textit{h r t.}"$. We create an embedding space by using an embedding model $M$ to create KG databases from verbalized triples. Each step is embedded in the space and searches $top\_k$ triples which are $top\_k$ highest probabilities of similarity of the step. With each considered triple, we calculate the ratio of overlap of head and tail entities with the step, which aims to evaluate if both entities exist in the step or not. To calculate, we utilize the function $partio\_ratio$ of FuzzyWuzzy library\footnote{https://pypi.org/project/fuzzywuzzy/}. Then, the $top\_k$ triples are re-ranked based on the average of all components including search probability $P$ as the relation score, overlap score of head entity $H$, and overlap score of tail entity $I$. The triple with the highest average score is considered as the best triple which represents the step.

As a result, after this step, we transformed LLM response $A =<(s_1,s_2,...s_n), a>$ into a reasoning path $\mathcal{P}=<T_1, T_2, ...>$. The framework continues to evaluate this reasoning path in the next stage.

\subsubsection{Reasoning path Validation}\label{path_eval}
While prior research only checks the factuality to verify a LLM answer \citep{chen2023felm, wang2023boosting}, our framework 
evaluates a reasoning path comprising 2 steps: fact-checking and relation-checking. The level of match and edit is checked for fine-grained evaluation.

\input{algos/algo-eval} 

\cref{algo:eval} depicts the algorithm to evaluate the validity of a reasoning path $\mathcal{P}$ with given thresholds. The thresholds of search probability and entities overlap are given as the best arguments by the evaluation of our framework in section \ref{sec:human_eval}.

For the fact-checking, a given reasoning path $\mathcal{P}=<T_1, T_2, ..., T_n>$,  is error if $\exists T_i < thresshold$, especially search probability $p$ < the threshold of search probability $\alpha$ and overlap of entities $h$,$t$ < threshold of entity overlap $\beta$. The relation-checking step is considered when all of the triples are fact and is evaluated by the connectivity in the triplets. We utilize the NetworkX library\footnote{https://pypi.org/project/networkx/} to construct and evaluate the connectivity given by the reasoning path. A reasoning path is only correct when guaranteeing all of the factual steps and creating a connected graph. Through \cref{algo:eval}, the factor leading to the invalidation of a reasoning path is figured out. 

\input{algos/algo_edit_eval}

For fine-grained reasoning path validation, we propose \cref{algo:eval_groundtruth} to check the alignment between the reasoning path with ground truth paths, leading to finding out the match rate and edit rate. Needleman Wunsch algorithm \citep{needleman1970general} is utilized for the alignment. Due to multiple ground truth reasoning path existence, we get the maximum match rate.



\subsection{Evaluation Metrics}\label{Evaluation}
In addition to the accuracy of the final answers, we aim to verify the correctness of the reasoning process. Specifically, we provide multi-facet metrics to assess the reasoning performance of LLMs. 

It is noticeable that a multitude of LLMs employed guardrail techniques to robust correctness, truthfulness, and faithfulness which return an abstained answer (e.g., “there is not enough information available to determine the answer.”). The detail of abstained answer detection is shown in Appendix \ref{appendix:abstained}. Furthermore, LLMs show different capabilities of the CoT instruction following, which return the correct format of a defined CoT response. The unstructured rate denotes the capability of LLM of CoT instruction following. The detail of unstructured answer detection is shown in Appendix \ref{appendix:unstructured}. So we define precision as the accuracy of non-abstained and structured answers 
\begin{equation}P=\frac{correct}{correct+incorrect}\end{equation} 
and recall as the accuracy of all answers 
\begin{equation}
  \resizebox{.5 \textwidth}{!} 
{
    $ R=\frac{correct}{correct+incorrect+abstained+unstructured} $
}
\end{equation}

The F1\_score 
\begin{equation}\label{equa:f1}F1 = 2×\frac{P*R}{P+R}\end{equation} is the main evaluation metric to compare the performance of LLMs.

\paragraph{Answer F1 score} is the accuracy of the final answers, using F1\_score shown in equation \ref{equa:f1}. Due to extracting from LLM generation, the final answers are a variety of lengths and LLM knowledge, we utilized a fuzzy match metric to check the correctness of the final answer. The fuzzy match metric checks if the generated final answer appears in the ground truth answers and vice versa. 

\paragraph{Reasoning F1 score} is the accuracy of the reasoning path, using F1\_score shown in equation \ref{equa:f1}. 
The method of checking the correctness of reasoning paths is shown in \cref{algo:eval}. A reasoning path is correct if \cref{algo:eval} returns \texttt{False} and vice versa.

% \paragraph{Confusion matrix} 
% \citet{Wei2022ChainThoughtPrompting} demonstrated that several LLM answers return correct answers but incorrect rationale. In this work, we examine the correlation between the correctness of reasoning and answers using confusion matrixes. The examination aims to answer the question: \textit{\textbf{Does a correct answer always cooperate with correct reasoning and vice versa?}} By providing evaluation results of reasoning and answer in part \ref{subsec:gen-cert}, we use confusion matrix function supported by Sklearn\footnote{https://scikit-learn.org} to explore the correlation of the final answer and reasoning. The order of required arguments of function in this case is the same.

==> sections/appx/appx-addtional-result.tex <==
\section{Additional Analysis}

\subsection{Figure 3}

\subsection{The relation path in CoT-Plan could elicit the 463
reasoning knowledge of LLMs and improve the 464
CoT reasoning.}

\subsection{Self-consistent can improve the trustfulness of 466
CoT reasoning by majority voting.}

\subsection{The higher the number of reasoning steps, the 468
lower trustfulness in CoT reasoning. }


==> table/decoding_strategy_eval.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\multirow{2}{*}{\textbf{Strategies}} & \multicolumn{2}{c}{\textbf{CWQ}} & \multicolumn{2}{c}{\textbf{GrailQA}}\\
\cmidrule(l){2-5} 
 & Answer & Reasoning & 
Answer & Reasoning\\
\midrule 
greedy & 51.83 & 33.8 & 25.14 & 4.71\\
temp=0.3, topp=1 & 51.86 & 32.68 & \textbf{25.57} & \textbf{5.60}\\
temp=0.5, topp=1 & 52.93 & \textbf{34.80} & 24.08 & 4.53\\
temp=0.7, topp=1 & 51.30 & 34.78 & 23.89 & 4.23\\
temp=1, topp=0.95 & \textbf{53.60} & 32.96 & 23.73 & 4.87\\
temp=0.7, topp=0.9 * & 52.40 & 33.66 & 24.75 & 4.47\\
\hline
\end{tabular}
}
\caption{Ablation study. The F1 score of ChatGPT's generative evaluation for various decoding strategies. Greedy denotes temp=0, topp=1. * denotes the default hyperparameters used for the main result. The best performance is shown in \textbf{bold}}
\label{tab:decoding_eval}
\end{table}


==> table/finegrained_match_edit.tex <==

\begin{table}
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc@{}}  % repeats {c|} 18 times
\toprule
\multirow{2}{*}{LLMs} & \multirow{2}{*}{Size} & \multicolumn{2}{c|}{\textbf{CWQ}} & \multicolumn{2}{c}{\textbf{GrailQA}}\\
\cmidrule(l){3-6} 
 &  & \multicolumn{1}{c}{Match} & Edit & 
\multicolumn{1}{c}{Match} & \multicolumn{1}{c}{Edit}\\
\midrule 
 Mistral & 7B & 27.09 & 69.86 & 6.44 & 94.03\\ 
 Qwen & 7B & 22.14 & 76.78 & 6.87 & 94.09\\
 Qwen  & 14B &  23.67 & 74.49 & 8.59 & 92.9\\
 Vicuna & 33B &  23.59 & 76.4 & 6.55 & 95.39\\
LLaMA2 & 70B & 34.55 & 62.23 & 8.08 & 92.58 \\
ChatGPT & 175B & \textbf{41.12} & \textbf{55.94} & \textbf{10.03} & \textbf{90.13} \\  
 \bottomrule
\end{tabular}
}
\caption{
The fine-grained result of the match rate and the edit rate of LLMs using the fewshot CoT prompt on CWQ and GrailQA datasets. The higher match rate is better, otherwise, the lower edit rate is better. The best performance is shown in \textbf{bold}.
}
\label{tab:fine-grained-eval}
\end{table}


==> table/generative_cert_main_old.tex <==
\begin{table*}[t!]
\centering
%\small
\resizebox{.88\textwidth}{!}{%
\begin{tabular}{@{}l|r|rrrr|rrrr@{}}  % repeats {c|} 18 times
\toprule
\multirow{2}{*}{LLMs} & \multirow{2}{*}{Size} & \multicolumn{4}{c}{\textbf{CWQ}} & \multicolumn{4}{c}{\textbf{GrailQA}}\\
% \cmidrule(l){3-10} 
 &  & \multicolumn{1}{c}{Answer$\uparrow$} & Reasoning$\uparrow$ & \multirow{1}{*}{Gap$\downarrow$} & \multirow{1}{*}{Edit Dist.$\downarrow$} & 
\multicolumn{1}{c}{Answer$\uparrow$} & \multicolumn{1}{c}{Reasoning$\uparrow$} & \multirow{1}{*}{Gap$\downarrow$} & \multirow{1}{*}{Edit Dist.$\downarrow$}\\
\midrule 
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{F1} & &
% \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{F1} &\\
% \hline 
& & \multicolumn{8}{c}{Fewshot CoT} \\  
\midrule 
 \texttt{Mistral} & 7B & \multicolumn{1}{c}{36.67} & 14.43 & \multicolumn{1}{c}{22.24} & 69.86 & 15.97 & 2.69 & 13.28 & 94.03\\ %\hline
  \texttt{Qwen} & 7B & \multicolumn{1}{c}{29.38} & 15.81 & \multicolumn{1}{c}{13.57} & 76.78 & 7.73 & 0.64 & 7.09 & 94.69\\
  \texttt{Qwen}  & 14B & \multicolumn{1}{c}{38.38} & 20.02 & \multicolumn{1}{c}{18.36} & 74.49 & 15.37 & 2.84 & 12.53 & 92.90\\
  \texttt{Vicuna} & 33B & \multicolumn{1}{c}{23.47} & 12.54 & \multicolumn{1}{c}{\textbf{10.93}} & 74.60 & 8.09 & 1.22 & \textbf{6.87} & 95.39\\ %\hline
 \texttt{LLaMA2} & 70B & \multicolumn{1}{c}{49.26} & 27.92 & \multicolumn{1}{c}{21.34} & 62.23 & 21.82 & 3.53 & 18.29 & 92.58\\ %\hline
 \texttt{ChatGPT} & 175B & \multicolumn{1}{c}{\textbf{52.40}} & \textbf{33.66} & \multicolumn{1}{c}{18.74} & \textbf{55.94} & \textbf{24.75} & \textbf{4.47 }& 20.28 & \textbf{90.13}\\  \midrule

& & \multicolumn{6}{c}{Fewshot CoT - Plan} \\ 
\midrule
  \texttt{Mistral} & 7B & \multicolumn{1}{c}{37.11\fontsize{6}{1}\selectfont \textcolor{black}{+0.44}} & 23.11\fontsize{6}{1}\selectfont \textcolor{black}{+0.87} & \multicolumn{1}{c}{\textbf{14.00}} & 70.01 & 17.66\fontsize{6}{1}\selectfont \textcolor{black}{+1.69} & 3.19\fontsize{6}{1}\selectfont \textcolor{black}{+0.5} & 14.47 & 94.46\\
  \texttt{Qwen}  & 7B & \multicolumn{1}{c}{35.47\fontsize{6}{1}\selectfont \textcolor{black}{+6.09}} & 17.81\fontsize{6}{1}\selectfont \textcolor{black}{+2.00} & \multicolumn{1}{c}{17.66} & 74.74 & 13.76\fontsize{6}{1}\selectfont \textcolor{black}{+6.03} & 2.47\fontsize{6}{1}\selectfont \textcolor{black}{+1.83} & \textbf{11.29} & 94.61\\
  \texttt{Qwen}  & 14B & \multicolumn{1}{c}{39.51\fontsize{6}{1}\selectfont \textcolor{black}{+1.13}} & 19.30\fontsize{6}{1}\selectfont \textcolor{black}{+0.19} & \multicolumn{1}{c}{20.21} & 73.68 & 16.98\fontsize{6}{1}\selectfont \textcolor{black}{+1.61} & 3.75\fontsize{6}{1}\selectfont \textcolor{black}{+0.91} & 13.23 & 92.58\\
  \texttt{Vicuna} & 33B & \multicolumn{1}{c}{43.25\fontsize{6}{1}\selectfont \textcolor{black}{+19.78}} & 
 24.58{\fontsize{6}{1}\selectfont \textcolor{black}{+12.04}}
 & \multicolumn{1}{c}{18.67} & 63.93 & 
 19.86{\fontsize{6}{1}\selectfont \textcolor{black}{+11.77}}
 & 5.04\fontsize{6}{1}\selectfont \textcolor{black}{+3.82} & 14.82 & 92.12\\
 \texttt{LLaMA2}  & 70B & 
\multicolumn{1}{c}{49.61{\fontsize{6}{1}\selectfont \textcolor{black}{+0.35}}}
& 
34.54{\fontsize{6}{1}\selectfont \textcolor{black}{+6.62}}
 & \multicolumn{1}{c}{15.07} & 57.81 &
22.25{\fontsize{6}{1}\selectfont \textcolor{black}{+0.43} }
& 
5.28{\fontsize{6}{1}\selectfont \textcolor{black}{+1.75} }
& 16.97 & 89.61\\ 
 \texttt{ChatGPT} & 175B & \multicolumn{1}{c}{\textbf{53.25{\fontsize{6}{1}\selectfont \textcolor{black}{+0.85}}}} & \textbf{35.38{\fontsize{6}{1}\selectfont \textcolor{black}{+1.72}}} & \multicolumn{1}{c}{17.87} & \textbf{55.61} & \textbf{27.16{\fontsize{6}{1}\selectfont \textcolor{black}{+2.41}}} & \textbf{5.85{\fontsize{6}{1}\selectfont \textcolor{black}{+1.38}}} & 21.31 & \textbf{89.54}\\ 
 \midrule	
 
& & \multicolumn{6}{c}{Fewshot CoT - SC} \\ 
\midrule
  \texttt{Mistral}  & 7B & \multicolumn{1}{c}{39.61\fontsize{6}{1}\selectfont \textcolor{black}{+2.94}} & 27.61\fontsize{6}{1}\selectfont\textcolor{black}{+5.37} & \multicolumn{1}{c}{\textbf{12.00}} & 65.21 & 18.58{\fontsize{6}{1}\selectfont \textcolor{black}{+2.61}} & 3.98{\fontsize{6}{1}\selectfont \textcolor{black}{+1.29}} & 14.60 & 94.10\\
  \texttt{Qwen}  & 7B & \multicolumn{1}{c}{36.31\fontsize{6}{1}\selectfont\textcolor{black}{+6.93}} & 19.70\fontsize{6}{1}\selectfont \textcolor{black}{+3.89} & \multicolumn{1}{c}{16.61} & 74.24 & 14.49{\fontsize{6}{1}\selectfont \textcolor{black}{+6.76}} & 1.80{\fontsize{6}{1}\selectfont \textcolor{black}{+1.16}} & 12.69 & 94.35\\
  \texttt{Qwen}  & 14B & \multicolumn{1}{c}{42.25\fontsize{6}{1}\selectfont \textcolor{black}{+3.87}} & 24.12\fontsize{6}{1}\selectfont \textcolor{black}{+4.10} & \multicolumn{1}{c}{18.13} & 73.21 & 19.98{\fontsize{6}{1}\selectfont \textcolor{black}{+4.61}} & 4.29{\fontsize{6}{1}\selectfont \textcolor{black}{+1.45}} & 15.69 & 92.50\\
  \texttt{Vicuna} & 33B & \multicolumn{1}{c}{37.36\fontsize{6}{1}\selectfont \textcolor{black}{+13.89}} & 20.68\fontsize{6}{1}\selectfont \textcolor{black}{+8.14} & \multicolumn{1}{c}{16.68} & 66.17& 9.07{\fontsize{6}{1}\selectfont \textcolor{black}{+0.98}} & 1.34{\fontsize{6}{1}\selectfont \textcolor{black}{+0.12}f} & \textbf{7.73} & 94.23\\
 \texttt{LLaMA2} & 70B & \multicolumn{1}{c}{50.10\fontsize{6}{1}\selectfont \textcolor{black}{+0.84}} & 31.25\fontsize{6}{1}\selectfont \textcolor{black}{+3.33} & \multicolumn{1}{c}{18.85} & 58.55	& 22.68{\fontsize{6}{1}\selectfont \textcolor{black}{+0.86}} & 3.73{\fontsize{6}{1}\selectfont \textcolor{black}{+0.2}} & 18.95 & 91.50\\ 
 \texttt{ChatGPT} & 175B & \multicolumn{1}{c}{\textbf{55.16\fontsize{6}{1}\selectfont \textcolor{black}{+2.76}}} & \textbf{37.25{\fontsize{6}{1}\selectfont\textcolor{black}{+3.59}}} & \multicolumn{1}{c}{17.91} & \textbf{52.56} & \textbf{27.26{\fontsize{6}{1}\selectfont \textcolor{black}{+2.51}}} & \textbf{5.33{\fontsize{6}{1}\selectfont \textcolor{black}{+0.59}}} & 22.20 & \textbf{89.22}\\ 
 \bottomrule
\end{tabular}
}
\caption{
Generative evaluation performance of different LLMs on CWQ and GrailQA datasets. F1-scores of the final answer and reasoning accuracy are reported in \texttt{Answer} \texttt{Reasoning} respectively. The \texttt{Gap} column denotes the differences between \texttt{Answer} and \texttt{Reasoning}. The \texttt{Edit Dist.} denotes the edit distance metric described in \Cref{appendix:eval-metric}. \texttt{+x.xx} denotes the improvement in comparison to few-shot CoT.}
% Fewshot CoT using prompt \ref{fig:fewshot_cot_only_prompt} as the baseline result. Fewshot CoT - Hint uses prompt \ref{fig:fewshot_cot_hint_prompt} to explore the ability of relation decomposition of LLMs. Fewshot CoT - SC is the self-consistency technique that returns 4 distinct sequences from the fewshot CoT prompt. 
% The best performance for each dataset is marked in \textbf{bold}. The \texttt{Answer} and \texttt{Reasoning} columns denote the F1-score of the final answer and reasoning accuracy, respectively (higher is better). The \texttt{Gap} column denotes the differences between \texttt{Answer} and \texttt{Reasoning}. The \texttt{Edit Dist.} denotes the edit distance metric described in appendix \ref{appendix:eval-metric}. \texttt{+xxx} denotes the improvement in comparison to Fewshot CoT.}
\label{tab:generative-cert}
\vspace{-1em}
\end{table*}


==> table/human_annotation_data.tex <==
\begin{table*}[]
\centering
%\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllcc}
\rowcolor[HTML]{FFFF00} 
\textbf{Question}                                                                                        & \textbf{LLM Answer}                                                                                                                                                                                                  & \textbf{ground\_reasoning\_path}                                                                                                                                                                                                       & \multicolumn{1}{l}{\cellcolor[HTML]{FFFF00}\textbf{incorrect\_answer}} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFF00}\textbf{incorrect\_reasoning}} \\
What is the country where Sakara Gold Beer is made and what type of currency is used there?              & \begin{tabular}[c]{@{}l@{}}1. Sakara Gold Beer is made in Egypt.\\ 2. The currency used in Egypt is the Egyptian pound.\\ So the answer is (Egypt, Egyptian pound).\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}{[}{[}{[}'El Gouna Beverage Co. Sakara Gold', 'food.beer\_country\_region.beers\_from\_here', 'Egypt'{]},\\  {[}'Egypt', 'location.country.currency\_used', 'Egyptian pound'{]}{]}{]}\end{tabular}          & 0                                                                      & 0                                                                         \\
What county is the city that includes the Houston City Council as a part of their government located in? & \begin{tabular}[c]{@{}l@{}}1. The Houston City Council is a part of the government of the city of Houston.\\ 2. Houston is located in Harris County, Texas.\\ So the answer is (Harris County).\end{tabular}         & \begin{tabular}[c]{@{}l@{}}{[}{[}{[}'Houston City Council', 'government.government\_position\_held.governmental\_body', 'Houston'{]}, \\ {[}'Houston', 'location.hud\_county\_place.county', 'Montgomery County'{]}{]}{]}\end{tabular} & 1                                                                      & 1                                                                         \\
What is the currency in the country where the Brazilian cruzado is also used?                            & \begin{tabular}[c]{@{}l@{}}1. The Brazilian cruzado was the currency of Brazil from 1986 to 1989.\\ 2. Brazil is the country where the Brazilian cruzado was used.\\ So the answer is (Brazilian real).\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}{[}"Brazilian cruzado","location.country.currency\_formerly\_used","Brazil"{]},\\ {[}"Brazil","location.country.currency\_used","Brazilian real"{]}{]}\end{tabular}                                      & 1                                                                      & 0                                                                         \\
Where was the main artist featured in the Rihanna: Live in Concert Tour raised?                          & \begin{tabular}[c]{@{}l@{}}1. The main artist featured in the Rihanna: Live in Concert Tour is Rihanna.\\ 2. Rihanna was raised in Barbados.\\ So the answer is (Barbados).\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}{[}{[}"Rihanna: Live in Concert Tour","music.artist.concert\_tours","Rihanna"{]},\\ {[}"Rihanna","people.person.place\_of\_birth","Saint Michael Parish"{]}{]}\end{tabular}                                 & 0                                                                      & 1                                                                        
\end{tabular}
}
\caption{Four representative examples for human annotation dataset.
}
\label{tab:annotation_data}

\end{table*}

==> table/recall_gen_cert_old.tex <==

\begin{table}
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|c|cc|cc@{}}  % repeats {c|} 18 times
\toprule
\multirow{2}{*}{LLMs} & \multirow{2}{*}{Size} & \multicolumn{2}{c|}{\textbf{CWQ}} & \multicolumn{2}{c}{\textbf{GrailQA}}\\
\cmidrule(l){3-6} 
 &  & \multicolumn{1}{c}{Answer} & Reasoning & 
\multicolumn{1}{c}{Answer} & \multicolumn{1}{c}{Reasoning}\\
\midrule 
& & \multicolumn{4}{c}{Fewshot CoT} \\  
\midrule 
 Mistral & 7B & 35.53 & 21.55 & 14.08 & 2.37\\ 
 Qwen & 7B & 24.21 & 13.03  & 5.07 & 0.42\\
 Qwen  & 14B &  34.04 & 17.76 & 11.76 & 2.17\\
 Vicuna & 33B &  22.31 & 11.92 & 7.62 & 1.15\\
LLaMA2 & 70B & 48.47 & 27.47 & 20.86 & 3.37 \\
ChatGPT & 175B & 50.48 & 32.43 & 21.68 & 3.92\\  
\midrule
& & \multicolumn{4}{c}{Fewshot CoT - Plan} \\ 
\midrule
 Mistral & 7B & 36.05 & 22.45 & 16.65 & 3.01\\
 Qwen  & 7B & 33.59 & 16.86 & 11.66 & 2.09\\
 Qwen  & 14B & 35.65 & 18.23 & 13.59 & 3.00\\
 Vicuna & 33B & 42.21 & 23.99 & 18.46 & 4.68\\
LLaMA2  & 70B & 49.04 & 34.14 & 21.32 & 5.06\\ 
ChatGPT & 175B & 51.20 & 34.01 & 25.61 & 5.52\\ 
 \midrule
& & \multicolumn{4}{c}{Fewshot CoT - SC} \\ 
\midrule
 Mistral  & 7B & 39.41 & 27.47 & 18.20 & 3.90\\
 Qwen  & 7B & 34.99 & 18.98 & 12.71 & 1.58\\
 Qwen  & 14B & 40.33 & 23.02 & 18.12 & 3.89\\
 Vicuna & 33B & 37.10 & 20.53 & 8.97 & 1.33\\
LLaMA2 & 70B & 49.81 & 31.07 & 22.28 & 3.66\\ 
ChatGPT & 175B & 54.16 & 36.58 & 25.53 & 4.74\\ 
 \bottomrule
\end{tabular}
}
\caption{
The recall of LLMs on CWQ and GrailQA datasets.
}
\label{tab:recall_gen_cert}
\end{table}


==> table/relation_error_eval.tex <==
\begin{table*}[]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|c|ccc|ccc@{}}  % repeats {c|} 18 times
\toprule
\multirow{2}{*}{LLMs} & \multirow{2}{*}{Size} & \multicolumn{3}{c|}{\textbf{CWQ}} & \multicolumn{3}{c}{\textbf{GrailQA}}\\
\cmidrule(l){3-8} 
 &  & Fewshot CoT & Fewshot CoT - Hint & Fewshot CoT - SC &
Fewshot CoT & Fewshot CoT - Hint & Fewshot CoT - SC\\  
\midrule 
 Mistral & 7B & 2.31 & 4.46 & 2.69 & 5.71 &  10.04 & 6.08\\ 
 Qwen & 7B & 1.07 & 1.6  & 0.78 & 5.87 & 6.33 & 4.39\\
 Qwen  & 14B &  2.4 & 6.42 & 1.91 & 5.39 &  10.96 & 5.06\\
 Vicuna & 33B &  0.66 & 4.86 & 6.58 &2.34 & 8.49 & 8.94\\
LLaMA2 & 70B & 3.7 & 4.85 & 4.17 & 7.38  & 13.03 & 6.88\\
ChatGPT & 175B & 3.62 & 5.77 & 3.65 & 11.6 & 13.4 & 11.04\\  
 \bottomrule
\end{tabular}
}
\caption{
The ratio of reasoning error detection.
}
\label{tab:relation_error_eval}
\end{table*}






